The Global Structure of Molecular Clouds: I. Trends with Mass and Star Formation Rate

We introduce a model for the large-scale, global 3D structure of molecular clouds. Motivated by the morphological appearance of clouds in surface density maps, we model clouds as cylinders, with the aim of backing out information about the volume density distribution of gas and its relationship to star formation. We test our model by applying it to surface density maps for a sample of nearby clouds and find solutions that fit each of the observed radial surface density profiles remarkably well. Our most salient findings are that clouds with higher central volume densities are more compact and also have lower total mass. These same lower-mass clouds tend to have shorter gas depletion times, regardless of whether we consider their total mass or dense mass. Our analyses lead us to conclude that cylindrical clouds can be characterized by a universal structure that sets the timescale on which they form stars.

==> table_clouds.tex <==
\begin{table}\centering
\begin{center}
\begin{tabular}{l | c c c c }
\multicolumn{5}{c}{}\\
\tableline\tableline
Cloud           & Distance  & $l$ bounds  & $b$ bounds & Pixel Scale \\
name            & [pc]      & [$^\circ$]  & [$^\circ$]  & [pc] \\
\hline
  Ophiuchus     & 136   & $(-9,-2)$     & $(13,19)$     &  0.051 \\
  Corona        & 156   & $(-2.5,6.5)$  & $(-26,-16)$   &  0.048  \\
  Perseus       & 282   & $(155,162)$   & $(-27,-15)$   &  0.11 \\
  Orion A       & 426   & $(205,  217)$ & $(-21, -18.5)$&  0.14  \\
  Orion B       & 431   & $(201, 210)$  & $(-17.5, -13)$&  0.15  \\
  California    & 452   & $(155, 169)$  & $(-6,-10)$    &  0.16 \\
  MonR2         & 785   & $(211,219)$   & $(-15,-10)$   & 0.33  \\
  Rosette       & 1343  & $(203,210)$   & $(-4.5,0)$    & 0.48  \\
\end{tabular}
\end{center}
\caption{Cloud boundaries and distances.}
\label{tab:clouds}
\end{table}
